Learning Lexical Entries for Robotic Commands using Crowdsourcing

Robotic commands in natural language usually contain various spatial descriptions that are semantically similar but syntactically different. Mapping such syntactic variants into semantic concepts that can be understood by robots is challenging due to the high flexibility of natural language expressions. To tackle this problem, we collect robotic commands for navigation and manipulation tasks using crowdsourcing. We further define a robot language and use a generative machine translation model to translate robotic commands from natural language to robot language. The main purpose of this paper is to simulate the interaction process between human and robots using crowdsourcing platforms, and investigate the possibility of translating natural language to robot language with paraphrases.

==> related-work.tex <==
%\section{Related Work}

%Earliest work on incrementally learning a semantic grammar was introduced in \cite{DBLP:conf/acl/GavaldaW98}.  \citeauthor{chen2012fast} proposed an online learning method to extract lexicons paired with their planing sequence in the robot navigation task.  Recently  \citeauthor{DBLP:conf/acl/MisraTLS15} propose an approach to learn semantic lexicon for high-level verbs by levering the environment.  
%
%\cite{DBLP:conf/hcomp/GoldbergWK13}
%\cite{DBLP:conf/hcomp/NguyenWL15}
%\cite{DBLP:conf/hcomp/HladkaHL14}
